EEMARQ: Efficient Lock-Free Range Queries with Memory Reclamation

Multi-Version Concurrency Control (MVCC) is a common mechanism for achieving linearizable range queries in database systems and concurrent data-structures. The core idea is to keep previous versions of nodes to serve range queries, while still providing atomic reads and updates. Existing concurrent data-structure implementations, that support linearizable range queries, are either slow, use locks, or rely on blocking reclamation schemes. We present EEMARQ, the first scheme that uses MVCC with lock-free memory reclamation to obtain a fully lock-free data-structure supporting linearizable inserts, deletes, contains, and range queries. Evaluation shows that EEMARQ outperforms existing solutions across most workloads, with lower space overhead and while providing full lock freedom.

==> preliminaries.tex <==
\section{Preliminaries} \label{sec-preliminaries}

We use the basic asynchronous shared memory model from~\cite{herlihy1991wait}. The system consists of a set of executing threads, communicating through the shared memory. The shared memory is accessed by hardware-provided atomic operations, such as reads, writes, compare-and-swap (CAS) and wide-compare-and-swap (WCAS). The CAS operation receives an address of a memory word, an expected value and a new value. If the address content is equal to the expected value, it replaces it with the new value and returns true. Otherwise, it returns false. The WCAS does the same for two adjacent words in memory. 
%We say that a CAS (or WCAS) execution is successful if it returns true, and unsuccessful otherwise.
%
We say that a concurrent implementation is \textit{lock-free} if, given that the executing threads are run for a sufficiently long time, at least one thread makes progress. 
In addition, we use the standard correctness condition of \emph{linearizability} from~\cite{herlihy1990linearizability}. Briefly, any operation must take effect at some point (referred to as its \emph{linearizability point}) between its invocation and response.

A mapping data structure represents a map from a set of unique keys to their respective values. Each key-value pair is represented by a node, consisting typically of immutable key and value, and some other mutable fields (e.g., \textit{next} pointers).
The data-structure has an entry point (e.g., a linked-list head~\cite{harris2001pragmatic} or a tree root~\cite{natarajan2014fast}).
The physical insertion of a node is the act of making it reachable from the entry point, and the physical deletion of a node is its unlinking from the data-structure (making it unreachable from the entry point). 
Many concurrent data-structure implementations~\cite{wei2021constant,harris2001pragmatic,natarajan2014fast} also include a level of logical insertion and deletion between the physical ones. I.e., a reachable node does not necessarily represent a key-value pair which is currently in the map. 
